Automatic Operating Room Surgical Activity Recognition for Robot-Assisted Surgery

Automatic recognition of surgical activities in the operating room (OR) is a key technology for creating next generation intelligent surgical devices and workflow monitoring/support systems. Such systems can potentially enhance efficiency in the OR, resulting in lower costs and improved care delivery to the patients. In this paper, we investigate automatic surgical activity recognition in robot-assisted operations. We collect the first large-scale dataset including 400 full-length multi-perspective videos from a variety of robotic surgery cases captured using Time-of-Flight cameras. We densely annotate the videos with 10 most recognized and clinically relevant classes of activities. Furthermore, we investigate state-of-the-art computer vision action recognition techniques and adapt them for the OR environment and the dataset. First, we fine-tune the Inflated 3D ConvNet (I3D) for clip-level activity recognition on our dataset and use it to extract features from the videos. These features are then fed to a stack of 3 Temporal Gaussian Mixture layers which extracts context from neighboring clips, and eventually go through a Long Short Term Memory network to learn the order of activities in full-length videos. We extensively assess the model and reach a peak performance of 88% mean Average Precision.

==> 6_res.tex <==
\section{Experimental Results}

\begin{table*}[t]
	\centering
	\scriptsize
	\caption{\small{I3D fine-tuning results.}}
	\label{tab:i3d}
	\vspace{-10pt}
	\begin{tabular}{@{}lccccccccccc@{}}\toprule
		& \multicolumn{3}{c}{Random} & \phantom{abc}& \multicolumn{3}{c}{Procedure} &
		\phantom{abc} & \multicolumn{3}{c}{Surgeon}\\ \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
		& Prec. & Rec. & F1 && Prec. & Rec. & F1 && Prec. & Rec. & F1\\ \midrule
		
		Sterile preparation & 97.0$\pm$1.4 & 96.3$\pm$1.7 & 96.5$\pm$1.3 && 86.44 & 78.46 & 82.26 && 81.08 & 88.24 & 84.51 \\
		Patient roll in     & 91.3$\pm$3.4 & 91.0$\pm$5.4 & 90.8$\pm$3.4 && 77.94 & 80.3 & 79.1 && 85.0 & 75.0 & 79.69 \\
		Patient preparation & 75.8$\pm$3.0 & 78.3$\pm$3.2 & 770.$\pm$2.6 && 55.56 & 78.57 & 65.09 && 61.97 & 62.86 & 62.41 \\ 
		Robot roll up       & 92.8$\pm$2.4 & 92.8$\pm$2.1 & 92.8$\pm$1.3 && 88.14 & 83.87 & 85.95 && 85.94 & 82.09 & 83.97 \\
		Robot docking       & 75.5$\pm$6.0 & 80.3$\pm$2.6 & 77.5$\pm$2.6 && 76.19 & 50.0 & 60.38 && 60.29 & 60.29 & 60.29 \\ 
		Surgery             & 80.5$\pm$1.7 & 86.0$\pm$5.4 & 83.0$\pm$1.4 && 69.51 & 81.43 & 75.0 && 73.33 & 74.32 & 73.83 \\
		Robot undocking     & 84.0$\pm$2.4 & 72.5$\pm$6.2 & 77.8$\pm$4.2 && 75.0 & 72.86 & 73.91 && 68.18 & 62.50 & 65.22 \\ 
		Robot roll back     & 96.3$\pm$2.2 & 90.8$\pm$3.3 & 93.3$\pm$2.4 && 94.64 & 80.30 & 86.89 && 98.08 & 76.12 & 85.71 \\
		Patient close       & 77.8$\pm$1.0 & 79.3$\pm$2.2 & 78.5$\pm$0.6 && 69.44 & 69.44 & 69.44 && 67.16 & 62.5 & 64.75 \\
		Patient roll out    & 88.5$\pm$3.4 & 90.3$\pm$4.9 & 89.3$\pm$1.5 && 73.53 & 73.53 & 73.53 && 63.64 & 90.0 & 74.56 \\
		\bottomrule
	\end{tabular}
\end{table*}

% \begin{table*}[t]
% 	\centering
% 	\small
% 	\caption{}
% 	\label{tab:i3d}
% 	\begin{tabular}{@{}lccccc@{}}\toprule
% 		& \multicolumn{1}{c}{Precision} & &
% 		\multicolumn{1}{c}{Recall}& &
% 		\multicolumn{1}{c}{F1}\\
%         \midrule
%         Sterile preparation    & 0.970$\pm$0.014 && 0.963$\pm$0.017 && 0.965$\pm$0.013 \\
%         Patient roll in        & 0.913$\pm$0.034 && 0.910$\pm$0.054 && 0.908$\pm$0.034 \\
%         Patient preparation    & 0.758$\pm$0.030 && 0.783$\pm$0.032 && 0.770$\pm$0.026 \\
%         Robot roll up          & 0.928$\pm$0.024 && 0.928$\pm$0.021 && 0.928$\pm$0.013 \\
%         Robot docking          & 0.755$\pm$0.060 && 0.803$\pm$0.026 && 0.775$\pm$0.026 \\
%         Surgery                & 0.805$\pm$0.017 && 0.860$\pm$0.054 && 0.830$\pm$0.014 \\
%         Robot undocking        & 0.840$\pm$0.024 && 0.725$\pm$0.062 && 0.778$\pm$0.042 \\
%         Robot roll back        & 0.963$\pm$0.022 && 0.908$\pm$0.033 && 0.933$\pm$0.024 \\
%         Patient close          & 0.778$\pm$0.010 && 0.793$\pm$0.022 && 0.785$\pm$0.006 \\
%         Patient roll out       & 0.885$\pm$0.034 && 0.903$\pm$0.049 && 0.893$\pm$0.015 \\
% 		\bottomrule
% 	\end{tabular}
% 	\vspace{-12pt}
% \end{table*}

\begin{table*}[t]
	\centering
	\small
	\caption{Full-length surgical activity recognition results (mAP).}
	\label{tab:map}
	\begin{tabular}{@{}lccccc@{}}\toprule
		& \multicolumn{1}{c}{I3D} & &
		\multicolumn{1}{c}{I3D-LSTM} & &
		\multicolumn{1}{c}{I3D-TGM-LSTM}\\
        \midrule
        Random          & 62.16 $\pm$ 1.60 && \textbf{88.81 $\pm$ 1.30} && 88.75 $\pm$ 2.07 \\
        % OR split              & 36.91 && 58.40 && \textbf{63.47} \\
        Procedure    & 47.98 && 75.39 && \textbf{78.04} \\
        Surgeon      & 50.31 && 78.29 && \textbf{78.77} \\
		\bottomrule
	\end{tabular}
	\vspace{-12pt}
\end{table*}

\subsection{Fine-Tuned I3D}
Per class precision, recall, and F1-scores of our experiment is shown in Table~\ref{tab:i3d}. As it can be observed, when splitting the videos randomly, we can train a reliable clip recognition model. We performed 4 rounds of experiments, every time with a new random data split. The performance shows we can train a model with high precision, recall, and F1 scores while keep the standard deviation low.

When separating videos based on which OR they were captured in, the performance drops significantly (precision: 64.9, recall: 61.9, F1: 61.8 percent on average). The reason behind this observation is twofold: 1) the number of training videos is significantly less, 2) certain types of operations (e.g., Fundoplication, Lobectomy, Thymectomy) had no instance in OR1 dataset and were only seen in OR2. Due to these reasons, our clip recognition model is less robust compared to random split experiments.

Next, we test model's generalization power when dealing with novel procedure types. This split is more difficult when compared to random as the testing surgery categories were never seen during the training. Therefore, as shown in Table~\ref{tab:i3d} (and as expected) we observe that F1-scores drop in every class of activity, yet retaining an average F1 score of 75.15\%. 

Finally, when splitting the videos based on the surgeons, we observe the same trend as procedure type split. This confirms that I3D is able to maintain a decent performance when tested on unseen surgeons.


\subsection{Full-Length Surgical Activity Recognition}
As described in section \ref{sec:ar}, we can use the baseline I3D to perform activity recognition on full-length case videos. To do so, we feed clips (of 16 consecutive frames) to I3D. I3D then predicts the activities in all clips of the same video. The performance of this baseline, in mean Average Precision (mAP), is reported under the first column of Table~\ref{tab:map}. Not surprisingly, the trend is similar to our clip-level recognition experiments; the performance is higher when the data split has more training videos. The base I3D yields mAP of 36.91\% when we split the videos by the OR they were captured in. We do not report this number in the table simply because the train/test split ratio is significantly different than the other 3 data split schemes.

When comparing I3D to our full pipeline (I3D-LSTM), we see a significant boost in performance under every split scheme. This is expected as classification of clips are done within the context of other clips in the video and also order of activities are learned. Peak performance of \textbf{88.81} mAP on average was obtained on random split. In worst case scenario that happens on OR data split, I3D-LSTM reaches to 58.40 mAP, which is significantly higher than the base I3D.

Finally, we use a recent technique~\cite{tgm} and add a Temporal Gaussian Mixture (TGM) layer before our LSTM to model longer-term temporal information in the video. This layer learns temporal filters per class of activity and uses them to provide further context before making a classification decision. The features of this layer are concatenated with I3D features and are then fed to LSTM. I3D-TGM-LSTM reaches mAP of $63.47\%$ on OR split, and in general, we see that this layer is increasing the model's generalization capacity; it performs on-par with I3D-LSTM on random split, but outperforms it on all 3 other splits.

% Since this baseline 1) lacks global context when predicting the activity in a single clip and 2) does not learn order of activities, we use an LSTM unit on top of the backbone as shown in Figure~\ref{fig:app}. This model is train on full-length videos (refer to section~\ref{lstm}). Table~\ref{tab:map} shows that this model outperforms the base I3D by significant margin (over 34\% mAP in random split and 22\% in OR split). This is expected as classification of clips are done within the context of other clips in the video and also order of activities are learned.
